Internal dynamics of Abell 1240: a galaxy cluster with symmetric double radio relics

We aim to obtain new insights into the internal dynamics of the cluster Abell 1240, showing the presence of two roughly symmetric radio relics, separated by ~2 h_70^-1 Mpc. Our analysis is mainly based on redshift data for 145 galaxies and on new photometric data. We also use X-ray data from the Chandra archive and photometric data from the SDSS (DR7). We combine galaxy velocities and positions to select 89 cluster galaxies and analyze the internal dynamics of the Abell 1237 + Abell 1240 cluster complex. We estimate similar redshifts for Abell 1237 and Abell 1240, <z>=0.1935 and <z>=0.1948, respectively. For Abell 1237 we estimate velocity dispersion sigma_v~740 km/s and a mass M~6 10^14 h_70^-1 M_sun. For Abell 1240 we estimate a LOS sigma_v~870 km/s and a mass range M~0.9-1.9 10^15 h_70^-1 M_sun, which takes into account its complex dynamics. Abell 1240 is shown to have a bimodal structure with two galaxy clumps roughly defining the N-S direction, the same one defined by the elongation of its X-ray surface brightness and by the axis of symmetry of the relics. The two--body model agrees with the hypothesis that we are looking at a cluster merger occurred largely in the plane of the sky, with the two galaxy clumps separated by a rest-frame velocity difference V_rf~2000 km/s at a time of 0.3 Gyrs after the crossing core, while Abell 1237 is still infalling onto Abell 1240. Chandra archive data confirm the complex structure of Abell 1240 and allow us to estimate a global X-ray temperature T_X=6.0+-0.5 keV. In agreement with the findings from radio data, our results for Abell 1240 strongly support the "outgoing merger shocks" model to explain the presence of the relics.

==> tabm.tex <==
\begin{table}
        \caption[]{Virial quantities}
         \label{tabamm}
                $$
         \begin{array}{l r r r}
            \hline
            \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
\mathrm{System} &{\rm 1D}\sigma_{\rm v}&\mathrm{R_{vir}}&\mathrm{Mass(<R_{vir}}\\
&\mathrm{km\ s^{-1}}&\mathrm{Mpc}&10^{14}\msun\\ 
            \hline
            \noalign{\smallskip}
\mathrm{A1237} &750 &1.6& 6        \\
\mathrm{A1240N}&850 &1.9& 9        \\
\mathrm{A1240S}&850 &1.9& 9        \\
\mathrm{A1240} &1100&2.4&2\times 10\\
              \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            \hline
         \end{array}
         \end{table}








